Measurement of the Branching Fraction for B^0 --> a1(1260)+-pi-+ with 535 Million BBbar Pairs

We present a measurement of the branching fraction for the decay B^0->a1+(1260)pi- with a1+->pi+pi+pi- using a data sample containing 535x10^6 BBbar pairs collected with the Belle detector at the KEKB asymmetric-energy e+e- collider operating at the Upsilon(4S) resonance. We measure the branching fraction Br(B^0->a1+pi-)Br(a1+->pi+pi+pi-) = (14.9 +- 1.6 +- 2.3)x10^-6, where the first and second errors are statistical and systematic, respectively.

==> author-conf2007.tex <==
%%% Paper:    
%%% Journal:  Summer 2007 Conference Papers
%%% Draft #1 (written June 6, 2007)
%%% Contacts: 
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\affiliation{Budker Institute of Nuclear Physics, Novosibirsk}
\affiliation{Chiba University, Chiba}
\affiliation{University of Cincinnati, Cincinnati, Ohio 45221}
\affiliation{Department of Physics, Fu Jen Catholic University, Taipei}
\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, Gie\ss{}en}
\affiliation{The Graduate University for Advanced Studies, Hayama}
\affiliation{Gyeongsang National University, Chinju}
\affiliation{Hanyang University, Seoul}
\affiliation{University of Hawaii, Honolulu, Hawaii 96822}
\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba}
\affiliation{Hiroshima Institute of Technology, Hiroshima}
\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801}
\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing}
\affiliation{Institute of High Energy Physics, Vienna}
\affiliation{Institute of High Energy Physics, Protvino}
\affiliation{Institute for Theoretical and Experimental Physics, Moscow}
\affiliation{J. Stefan Institute, Ljubljana}
\affiliation{Kanagawa University, Yokohama}
\affiliation{Korea University, Seoul}
\affiliation{Kyoto University, Kyoto}
\affiliation{Kyungpook National University, Taegu}
\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne}
\affiliation{University of Ljubljana, Ljubljana}
\affiliation{University of Maribor, Maribor}
\affiliation{University of Melbourne, School of Physics, Victoria 3010}
\affiliation{Nagoya University, Nagoya}
\affiliation{Nara Women's University, Nara}
\affiliation{National Central University, Chung-li}
\affiliation{National United University, Miao Li}
\affiliation{Department of Physics, National Taiwan University, Taipei}
\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow}
\affiliation{Nippon Dental University, Niigata}
\affiliation{Niigata University, Niigata}
\affiliation{University of Nova Gorica, Nova Gorica}
\affiliation{Osaka City University, Osaka}
\affiliation{Osaka University, Osaka}
\affiliation{Panjab University, Chandigarh}
\affiliation{Peking University, Beijing}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\affiliation{Princeton University, Princeton, New Jersey 08544}
\affiliation{RIKEN BNL Research Center, Upton, New York 11973}
\affiliation{Saga University, Saga}
\affiliation{University of Science and Technology of China, Hefei}
\affiliation{Seoul National University, Seoul}
\affiliation{Shinshu University, Nagano}
\affiliation{Sungkyunkwan University, Suwon}
\affiliation{University of Sydney, Sydney, New South Wales}
\affiliation{Tata Institute of Fundamental Research, Mumbai}
\affiliation{Toho University, Funabashi}
\affiliation{Tohoku Gakuin University, Tagajo}
\affiliation{Tohoku University, Sendai}
\affiliation{Department of Physics, University of Tokyo, Tokyo}
\affiliation{Tokyo Institute of Technology, Tokyo}
\affiliation{Tokyo Metropolitan University, Tokyo}
\affiliation{Tokyo University of Agriculture and Technology, Tokyo}
\affiliation{Toyama National College of Maritime Technology, Toyama}
\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
\affiliation{Yonsei University, Seoul}
% \author{K.~Abe}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{I.~Adachi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{H.~Aihara}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{D.~Anipko}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{K.~Arinstein}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{T.~Aso}\affiliation{Toyama National College of Maritime Technology, Toyama} % Toyama
% \author{V.~Aulchenko}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{T.~Aushev}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{T.~Aziz}\affiliation{Tata Institute of Fundamental Research, Mumbai} % Tata
% \author{S.~Bahinipati}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{A.~M.~Bakich}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{V.~Balagura}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{Y.~Ban}\affiliation{Peking University, Beijing} % Peking
% \author{S.~Banerjee}\affiliation{Tata Institute of Fundamental Research, Mumbai} % Tata
% \author{E.~Barberio}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{A.~Bay}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{I.~Bedny}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{K.~Belous}\affiliation{Institute of High Energy Physics, Protvino} % Protvino
% \author{V.~Bhardwaj}\affiliation{Panjab University, Chandigarh} % Panjab
% \author{U.~Bitenc}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{S.~Blyth}\affiliation{National United University, Miao Li} % NUU
% \author{A.~Bondar}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{A.~Bozek}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{M.~Bra\v cko}\affiliation{University of Maribor, Maribor}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{J.~Brodzicka}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{T.~E.~Browder}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{M.-C.~Chang}\affiliation{Department of Physics, Fu Jen Catholic University, Taipei} % FuJen
% \author{P.~Chang}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{Y.~Chao}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{A.~Chen}\affiliation{National Central University, Chung-li} % NCU
% \author{K.-F.~Chen}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{W.~T.~Chen}\affiliation{National Central University, Chung-li} % NCU
% \author{B.~G.~Cheon}\affiliation{Hanyang University, Seoul} % Hanyang
% \author{C.-C.~Chiang}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{R.~Chistov}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{I.-S.~Cho}\affiliation{Yonsei University, Seoul} % Yonsei
% \author{S.-K.~Choi}\affiliation{Gyeongsang National University, Chinju} % Gyeongsang
% \author{Y.~Choi}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{Y.~K.~Choi}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{S.~Cole}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{J.~Dalseno}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{M.~Danilov}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{A.~Das}\affiliation{Tata Institute of Fundamental Research, Mumbai} % Tata
% \author{M.~Dash}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{J.~Dragic}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{A.~Drutskoy}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{S.~Eidelman}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{D.~Epifanov}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{S.~Fratina}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{H.~Fujii}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{M.~Fujikawa}\affiliation{Nara Women's University, Nara} % Nara
% \author{N.~Gabyshev}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{A.~Garmash}\affiliation{Princeton University, Princeton, New Jersey 08544} % Princeton
% \author{A.~Go}\affiliation{National Central University, Chung-li} % NCU
% \author{G.~Gokhroo}\affiliation{Tata Institute of Fundamental Research, Mumbai} % Tata
% \author{P.~Goldenzweig}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{B.~Golob}\affiliation{University of Ljubljana, Ljubljana}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{M.~Grosse~Perdekamp}\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % UIUC
% \author{H.~Guler}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{H.~Ha}\affiliation{Korea University, Seoul} % Korea
% \author{J.~Haba}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{K.~Hara}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{T.~Hara}\affiliation{Osaka University, Osaka} % Osaka
% \author{Y.~Hasegawa}\affiliation{Shinshu University, Nagano} % Shinshu
% \author{N.~C.~Hastings}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{K.~Hayasaka}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{H.~Hayashii}\affiliation{Nara Women's University, Nara} % Nara
% \author{M.~Hazumi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{D.~Heffernan}\affiliation{Osaka University, Osaka} % Osaka
% \author{T.~Higuchi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{L.~Hinz}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{H.~Hoedlmoser}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{T.~Hokuue}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{Y.~Horii}\affiliation{Tohoku University, Sendai} % Tohoku
% \author{Y.~Hoshi}\affiliation{Tohoku Gakuin University, Tagajo} % TohokuGakuin
% \author{K.~Hoshina}\affiliation{Tokyo University of Agriculture and Technology, Tokyo} % TUAT
% \author{S.~Hou}\affiliation{National Central University, Chung-li} % NCU
% \author{W.-S.~Hou}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{Y.~B.~Hsiung}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{H.~J.~Hyun}\affiliation{Kyungpook National University, Taegu} % Kyungpook
% \author{Y.~Igarashi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{T.~Iijima}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{K.~Ikado}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{K.~Inami}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{H.~Ishino}\affiliation{Tokyo Institute of Technology, Tokyo} % TIT
% \author{R.~Itoh}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{M.~Iwabuchi}\affiliation{The Graduate University for Advanced Studies, Hayama} % Sokendai
% \author{M.~Iwasaki}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{Y.~Iwasaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{C.~Jacoby}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{M.~Jones}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{N.~J.~Joshi}\affiliation{Tata Institute of Fundamental Research, Mumbai} % Tata
% \author{M.~Kaga}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{D.~H.~Kah}\affiliation{Kyungpook National University, Taegu} % Kyungpook
% \author{H.~Kaji}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{S.~Kajiwara}\affiliation{Osaka University, Osaka} % Osaka
% \author{H.~Kakuno}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{J.~H.~Kang}\affiliation{Yonsei University, Seoul} % Yonsei
% \author{P.~Kapusta}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{S.~U.~Kataoka}\affiliation{Nara Women's University, Nara} % Nara
% \author{N.~Katayama}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{H.~Kawai}\affiliation{Chiba University, Chiba} % Chiba
% \author{T.~Kawasaki}\affiliation{Niigata University, Niigata} % Niigata
% \author{A.~Kibayashi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{H.~Kichimi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{H.~J.~Kim}\affiliation{Kyungpook National University, Taegu} % Kyungpook
% \author{H.~O.~Kim}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{J.~H.~Kim}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{S.~K.~Kim}\affiliation{Seoul National University, Seoul} % Seoul
% \author{Y.~J.~Kim}\affiliation{The Graduate University for Advanced Studies, Hayama} % Sokendai
% \author{K.~Kinoshita}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{S.~Korpar}\affiliation{University of Maribor, Maribor}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{Y.~Kozakai}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{P.~Kri\v zan}\affiliation{University of Ljubljana, Ljubljana}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{P.~Krokovny}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{R.~Kumar}\affiliation{Panjab University, Chandigarh} % Panjab
% \author{E.~Kurihara}\affiliation{Chiba University, Chiba} % Chiba
% \author{A.~Kusaka}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{A.~Kuzmin}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{Y.-J.~Kwon}\affiliation{Yonsei University, Seoul} % Yonsei
% \author{J.~S.~Lange}\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, Gie\ss{}en} % Giessen
% \author{G.~Leder}\affiliation{Institute of High Energy Physics, Vienna} % Vienna
% \author{J.~Lee}\affiliation{Seoul National University, Seoul} % Seoul
% \author{J.~S.~Lee}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{M.~J.~Lee}\affiliation{Seoul National University, Seoul} % Seoul
% \author{S.~E.~Lee}\affiliation{Seoul National University, Seoul} % Seoul
% \author{T.~Lesiak}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{J.~Li}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{A.~Limosani}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{S.-W.~Lin}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{Y.~Liu}\affiliation{The Graduate University for Advanced Studies, Hayama} % Sokendai
% \author{D.~Liventsev}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{J.~MacNaughton}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{G.~Majumder}\affiliation{Tata Institute of Fundamental Research, Mumbai} % Tata
% \author{F.~Mandl}\affiliation{Institute of High Energy Physics, Vienna} % Vienna
% \author{D.~Marlow}\affiliation{Princeton University, Princeton, New Jersey 08544} % Princeton
% \author{T.~Matsumura}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{A.~Matyja}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{S.~McOnie}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{T.~Medvedeva}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{Y.~Mikami}\affiliation{Tohoku University, Sendai} % Tohoku
% \author{W.~Mitaroff}\affiliation{Institute of High Energy Physics, Vienna} % Vienna
% \author{K.~Miyabayashi}\affiliation{Nara Women's University, Nara} % Nara
% \author{H.~Miyake}\affiliation{Osaka University, Osaka} % Osaka
% \author{H.~Miyata}\affiliation{Niigata University, Niigata} % Niigata
% \author{Y.~Miyazaki}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{R.~Mizuk}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{G.~R.~Moloney}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{T.~Mori}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{J.~Mueller}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
% \author{A.~Murakami}\affiliation{Saga University, Saga} % Saga
% \author{T.~Nagamine}\affiliation{Tohoku University, Sendai} % Tohoku
% \author{Y.~Nagasaka}\affiliation{Hiroshima Institute of Technology, Hiroshima} % Hiroshima
% \author{Y.~Nakahama}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{I.~Nakamura}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{E.~Nakano}\affiliation{Osaka City University, Osaka} % OsakaCity
% \author{M.~Nakao}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{H.~Nakayama}\affiliation{Department of Physics, University of Tokyo, Tokyo} % Tokyo
% \author{H.~Nakazawa}\affiliation{National Central University, Chung-li} % NCU
% \author{Z.~Natkaniec}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{K.~Neichi}\affiliation{Tohoku Gakuin University, Tagajo} % TohokuGakuin
% \author{S.~Nishida}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{K.~Nishimura}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{Y.~Nishio}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{I.~Nishizawa}\affiliation{Tokyo Metropolitan University, Tokyo} % TMU
% \author{O.~Nitoh}\affiliation{Tokyo University of Agriculture and Technology, Tokyo} % TUAT
% \author{S.~Noguchi}\affiliation{Nara Women's University, Nara} % Nara
% \author{T.~Nozaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{A.~Ogawa}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % RIKEN
% \author{S.~Ogawa}\affiliation{Toho University, Funabashi} % Toho
% \author{T.~Ohshima}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{S.~Okuno}\affiliation{Kanagawa University, Yokohama} % Kanagawa
% \author{S.~L.~Olsen}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{S.~Ono}\affiliation{Tokyo Institute of Technology, Tokyo} % TIT
% \author{W.~Ostrowicz}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{H.~Ozaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{P.~Pakhlov}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{G.~Pakhlova}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{H.~Palka}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{C.~W.~Park}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{H.~Park}\affiliation{Kyungpook National University, Taegu} % Kyungpook
% \author{K.~S.~Park}\affiliation{Sungkyunkwan University, Suwon} % Sungkyunkwan
% \author{N.~Parslow}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{L.~S.~Peak}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{M.~Pernicka}\affiliation{Institute of High Energy Physics, Vienna} % Vienna
% \author{R.~Pestotnik}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{M.~Peters}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{L.~E.~Piilonen}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{A.~Poluektov}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{J.~Rorie}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{M.~Rozanska}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{H.~Sahoo}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{Y.~Sakai}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{H.~Sakamoto}\affiliation{Kyoto University, Kyoto} % Kyoto
% \author{H.~Sakaue}\affiliation{Osaka City University, Osaka} % OsakaCity
% \author{T.~R.~Sarangi}\affiliation{The Graduate University for Advanced Studies, Hayama} % Sokendai
% \author{N.~Satoyama}\affiliation{Shinshu University, Nagano} % Shinshu
% \author{K.~Sayeed}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{T.~Schietinger}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{O.~Schneider}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{P.~Sch\"onmeier}\affiliation{Tohoku University, Sendai} % Tohoku
% \author{J.~Sch\"umann}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{C.~Schwanda}\affiliation{Institute of High Energy Physics, Vienna} % Vienna
% \author{A.~J.~Schwartz}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{R.~Seidl}\affiliation{University of Illinois at Urbana-Champaign, Urbana, Illinois 61801}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % UIUC
% \author{A.~Sekiya}\affiliation{Nara Women's University, Nara} % Nara
% \author{K.~Senyo}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{M.~E.~Sevior}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{L.~Shang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing} % IHEP
% \author{M.~Shapkin}\affiliation{Institute of High Energy Physics, Protvino} % Protvino
% \author{C.~P.~Shen}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing} % IHEP
% \author{H.~Shibuya}\affiliation{Toho University, Funabashi} % Toho
% \author{S.~Shinomiya}\affiliation{Osaka University, Osaka} % Osaka
% \author{J.-G.~Shiu}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{B.~Shwartz}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{V.~Sidorov}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{J.~B.~Singh}\affiliation{Panjab University, Chandigarh} % Panjab
% \author{A.~Sokolov}\affiliation{Institute of High Energy Physics, Protvino} % Protvino
% \author{A.~Somov}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{S.~Stani\v c}\affiliation{University of Nova Gorica, Nova Gorica} % NovaGorica
% \author{M.~Stari\v c}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{A.~Sugiyama}\affiliation{Saga University, Saga} % Saga
% \author{K.~Sumisawa}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{T.~Sumiyoshi}\affiliation{Tokyo Metropolitan University, Tokyo} % TMU
% \author{S.~Suzuki}\affiliation{Saga University, Saga} % Saga
% \author{S.~Y.~Suzuki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{O.~Tajima}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{F.~Takasaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{K.~Tamai}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{N.~Tamura}\affiliation{Niigata University, Niigata} % Niigata
% \author{M.~Tanaka}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{N.~Taniguchi}\affiliation{Kyoto University, Kyoto} % Kyoto
% \author{G.~N.~Taylor}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{Y.~Teramoto}\affiliation{Osaka City University, Osaka} % OsakaCity
% \author{I.~Tikhomirov}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{K.~Trabelsi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{Y.~F.~Tse}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{T.~Tsuboyama}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{K.~Uchida}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{Y.~Uchida}\affiliation{The Graduate University for Advanced Studies, Hayama} % Sokendai
% \author{S.~Uehara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{K.~Ueno}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{T.~Uglov}\affiliation{Institute for Theoretical and Experimental Physics, Moscow} % ITEP
% \author{Y.~Unno}\affiliation{Hanyang University, Seoul} % Hanyang
% \author{S.~Uno}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{P.~Urquijo}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{Y.~Ushiroda}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{Y.~Usov}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{G.~Varner}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{K.~E.~Varvell}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{K.~Vervink}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{S.~Villa}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{A.~Vinokurova}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{C.~C.~Wang}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{C.~H.~Wang}\affiliation{National United University, Miao Li} % NUU
% \author{J.~Wang}\affiliation{Peking University, Beijing} % Peking
% \author{M.-Z.~Wang}\affiliation{Department of Physics, National Taiwan University, Taipei} % Taiwan
% \author{P.~Wang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing} % IHEP
% \author{X.~L.~Wang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing} % IHEP
% \author{M.~Watanabe}\affiliation{Niigata University, Niigata} % Niigata
% \author{Y.~Watanabe}\affiliation{Kanagawa University, Yokohama} % Kanagawa
% \author{R.~Wedd}\affiliation{University of Melbourne, School of Physics, Victoria 3010} % Melbourne
% \author{J.~Wicht}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
% \author{L.~Widhalm}\affiliation{Institute of High Energy Physics, Vienna} % Vienna
% \author{J.~Wiechczynski}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow} % Krakow
% \author{E.~Won}\affiliation{Korea University, Seoul} % Korea
% \author{B.~D.~Yabsley}\affiliation{University of Sydney, Sydney, New South Wales} % Sydney
% \author{A.~Yamaguchi}\affiliation{Tohoku University, Sendai} % Tohoku
% \author{H.~Yamamoto}\affiliation{Tohoku University, Sendai} % Tohoku
% \author{M.~Yamaoka}\affiliation{Nagoya University, Nagoya} % Nagoya
% \author{Y.~Yamashita}\affiliation{Nippon Dental University, Niigata} % NihonDental
% \author{M.~Yamauchi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
% \author{C.~Z.~Yuan}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing} % IHEP
% \author{Y.~Yusa}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{C.~C.~Zhang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing} % IHEP
% \author{L.~M.~Zhang}\affiliation{University of Science and Technology of China, Hefei} % USTC
% \author{Z.~P.~Zhang}\affiliation{University of Science and Technology of China, Hefei} % USTC
% \author{V.~Zhilich}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{V.~Zhulanov}\affiliation{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
% \author{A.~Zupanc}\affiliation{J. Stefan Institute, Ljubljana} % Ljubljana
% \author{N.~Zwahlen}\affiliation{Swiss Federal Institute of Technology of Lausanne, EPFL, Lausanne} % Lausanne
\collaboration{The Belle Collaboration}


==> diff.tex <==
---
> \noaffiliation
469,471c117,118
< Recently, the BaBar collaboration reported the first measurement
< of the branching fraction
< of $B^0\to\aonepi$ assuming a 50\% branching fraction for
---
> Recently the BaBar collaboration first measured the branching fraction
> of $B^0\to\aonepi$ with an assumption of a 50\% branching fraction for
482c129
< The value of $\phi_2$ can be extracted using the method
---
> The $\phi_2$ value can be extracted using the method
499c146
< and $\pi^+\pi^-\pi^+\pi^-$ decays are neglected in the nominal fit.
---
> and $\pi^+\pi^-\pi^+\pi^-$ decays are neglected for the nominal fit.
501c148
< to the three pion mass distribution
---
> to the three pion mass distribution,
558c205
< We explicitly eliminate three charm $B$ decay modes that peak
---
> We explicitly eliminate three charm $B$ decay modes that make a peak
597c244
< are included for each event selected from the data. 
---
> are included for each event selected from the data sample.
641,643c288,290
< are obtained from a large MC sample and 
< modeled as two-dimensional smoothed histograms for $\de$-$\mbc$
< and polynomial functions for $\cos\theta$.
---
> are modeled as two-dimensional smoothed histograms for $\de$-$\mbc$
> and polynomial functions for $\cos\theta$
> obtained from a large MC sample.
694c341
< the $\de$, $\mbc$ and $\cos\theta$ distributions with
---
> $\de$, $\mbc$ and $\cos\theta$ distributions with
713c360
< We calculate the product of the branching fractions using
---
> We calculate a product of the branching fractions using
721,722c368,369
< $\aone\to\rho^0\pi^{\pm}$ decay vi an $S$-wave.
< The correction factor $\varepsilon_{\rm PID}=0.90$ 
---
> $\aone\to\rho^0\pi^{\pm}$ decay, $S$-wave.
> $\varepsilon_{\rm PID}=0.90$ is the correction factor that
725,726c372
< a large sample of $D^{*+}\to D^{0}\pi^{+}$, $D^{0}\to K^-\pi^+$ decays
< in data.
---
> a large data sample of $D^{*+}\to D^{0}\pi^{+}$, $D^{0}\to K^-\pi^+$ decays.
742c388
< No bias is found in the fits to pseudo-experiment samples.
---
> No bias is found for the fit to pseudo-experiment samples.
749c395
< from an unbinned maximum likelihood fit to
---
> by applying an unbinned maximum likelihood fit to
802c448
< generated assuming three- and four-body phase space distributions;
---
> generated assuming three and four body phase space distributions;
818,819c464,465
< originates from the uncertainty in the non-resonant contributions,
< which corresponds to a $\pm 11$\% systematic error.
---
> originates from the uncertainty in the non-resonant contributions.
> We assign a $\pm 11$\% systematic error.
824c470
< the uncertainties in the $\aone$ decays into 
---
> the uncertainties of the $\aone$ decays into 

